Circularization in the damped Kepler problem

In this paper, we revisit the damped Kepler problem within a general family of nonlinear damping forces with magnitude $\delta \vert u\vert^{\beta}\vert \dot u\vert^{\alpha+1}$, depending on three parameters $\delta>0,\alpha\ge 0$ and $\beta\ge 0$, and address the general question of circularization whereby orbits tend to become more circular as they approach the sun. Our approach is based on dynamical systems theory, using blowup and desingularization as our main technical tools. We find that $\gamma=\alpha+2\beta-3$ is an important quantity, with the special case $\gamma=0$ separating circularization ($-3<\gamma<0$) where the eccentricity converges to zero, i.e. $e(t)\rightarrow 0$ as $u(t)\rightarrow 0$, from cases ($\gamma>0$) where $e(t)\rightarrow 1$ as $u(t)\rightarrow 0$, both on open sets of initial conditions. We find that circularization for $-3<\gamma<0$ occurs due to asymptotic stability of a zero-Hopf equilibrium point (i.e., the eigenvalues are $\pm i \omega,0$) of a three-dimensional reduced problem (which is analytic in the blowup coordinates). The attraction is therefore not hyperbolic and in particular not covered by standard dynamical systems theory. Instead we use recent results on normal forms of the zero-Hopf to locally bring the system into a form where the stability can be addressed directly. We believe that our approach can be used to describe unbounded solutions.

==> old.tex <==
\par
XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
In this paper, we consider the damped Kepler problem \cite{margheri2014a,margheri2017a}
%\begin{align}
% \ddot u +\Delta(u,\dot u) \dot u + \frac{u}{\vert u\vert^3}=0,\eqlab{keplerd}
%\end{align}
with $u(t)\in \mathbb R^2\backslash \{0\}$ and where the damping function $\Delta$ takes the following general form
%\begin{align}
% \Delta(u,\dot u) = \delta \frac{\vert \dot u\vert^\alpha}{\vert %u\vert^\beta},\quad \alpha,\beta\ge 0,\quad \delta>0.\eqlab{Dfunc}
%\end{align}
(Notice in comparison with \cite{margheri2020a}, that we have replaced their $\alpha$ by $\alpha+1$.)
% Although our approach does generalize to other (rational) values, we will for simplicity restrict attention to $(\alpha,\beta)\in \mathbb N_0^2$. 
The case $(\alpha,\beta)=(0,0)$ corresponds to linear damping, also referred to as Stokes drag, and has been studied by many authors, see e.g. \cite{}. Also the case $(\alpha,\beta)=(0,2)$, known as the Poynting-Plummer-Danby drag, has also been studied previously, see \cite{}. Finally, the reference \cite{} considered the cases $(\alpha,\beta)\in \{0\}\times \mathbb R_{+}$. [TBD: summary and highlight not complete description. ] In this paper, we follow the blowup approach used in \cite{} to study all cases. 

The interest in the damped Kepler problem \eqref{keplerd} with $\Delta$ given by \eqref{Dfunc} dates back to Poincar\'e, see \cite{}. He found that orbits with negative energy $E(u,\dot u)<0$, where
\begin{align*}
 E(u,\dot u):= \frac{1}{2}\vert \dot u\vert^2-\frac{1}{\vert u\vert},
\end{align*}
spiral toward the singularity/collision limit $u=0$, doing so with increasing velocity. [TBD: explain argument of Poincare and why it is insufficient.] Moreover, he claimed that for $\alpha$ and $\beta$ large enough, orbits would tend to \textit{circularize}, in the sense that the eccentricity vector:
% \begin{align*}
%  he eccentricity vector
\begin{align*}
 \mathcal E(u,\dot u) = \dot u \wedge L(u,\dot u)-\frac{u}{\vert u\vert}
\end{align*}
% \end{align*}
with $L$ being the angular momentum
\begin{align*}
 L(u,\dot u)=u\wedge \dot u,
\end{align*}
approaches $0$ as $t\rightarrow \infty$.




It is known that circularization \textit{does not occur} for the linear damping (Stokes drag) $(\alpha,\beta)=(0,0)$ nor for the PPD case $(\alpha,\beta)=(0,2)$, see \cite{}. In particular, in the case of linear damping, then $\mathcal E(u,\dot u)\rightarrow 0$ only on a submanifold, see \cite{}. 



\note{Need something on the use of blowup in general: (Copy-pasted from a separate manuscript of mine)} 

Consider a vector-field $V$ in $\mathbb R^n$ having a fully nonhyperbolic singularity at the origin with the linearization having only zero eigenvalues. A blowup transformation $\Phi$ is then a weighted (or quasihomogeneous \cite{kuehn2015}), transformation of the form
\begin{align*}
\Phi:\,[0,\infty)\times S^{n-1}\rightarrow \mathbb R^n:\, (\rho,\bar{ x})\mapsto  x,\quad (\rho,\bar{x})\mapsto (\rho^{\kappa_1}\bar x_1,\ldots,\rho^{\kappa_n}\bar x_n),
\end{align*}
with the weights $\kappa$ chosen such that 
              \begin{align*}
               \widehat V:=\rho^{-k} \Phi^*(V),
              \end{align*}
              on $(\rho,\bar x)\in (0,\rho_0]\times S^{n-1}$, 
extends continuously/smoothly and nontrivially (\KUK{i.e. $\widehat V$ is not identically zero}) to $\rho=0$ for some $k\in \mathbb N$. The most useful situation is when the division by $\rho^{-k}$ (desingularization) leads to hyperbolicity of equilibria within $\rho=0$, so that the usual hyperbolic methods (linearization, stable, unstable and center manifolds, etc) of dynamical systems theory, see e.g. \KUK{\cite{perko2001a}}, can be applied. See also \cite[Chapter 3.3]{dumortier2006a} for general results on blowup (including the use of Newton polygons to select the weights) for planar systems. \KUK{expand this later:} It is also possible to blowup sets of degenerate singularities, see e.g. \cite{}.
XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\subsection{Overview}
\KUK{Something here, including: We emphasize that \secref{blowup} is introduced to motivate the coordinates; the analysis in \secref{gammaPos}, \secref{gammaNeg} and \secref{gammaEq0} can be read independently.}
\section{The notion of circularization}\seclab{circularization}
% 
%\note{I've changed this a bit. }
\RO{In principle the equation \eqref{keplerd} should be considered in the three dimensional space but a simple computation on the angular momentum 
$$L(u,\dot{u})=u\wedge \dot{u}$$
shows that }
\begin{align}
 \frac{d}{dt} L = -R(u,\dot u) L, \eqlab{Leqn}
\end{align}
and the direction of $L\in \mathbb R^3$ is therefore preserved. Consequently, as in the unperturbed Kepler problem, corresponding to $\delta=0$, the dynamics with $L\ne 0$ are confined to an orbital plane (with normal vector $L$) and for this reason, we will consider \eqref{keplerd} on the phase space
$$P:=(\mathbb{R}^2 \setminus \{ 0\} )\times \mathbb{R}^2 $$
\RO{with generic points $(x,v)$.}

